RELAY: Readout-Driven Early Stopping and Visual Relay for Multimodal Multi-Agent Reasoning

Multi-agent collaboration has become an effective test-time paradigm for complex reasoning in vision-language models (VLMs), yet existing methods execute a fixed chain of agents on every input regardless of question difficulty. On easy multimodal questions, running additional agents causes overthinking and wastes tokens; on hard questions, passing unfinished flawed reasoning text across agents accumulates and propagates early visual errors. To overcome both limitations, we propose RELAY (Readout-Driven Early Stopping and Visual Relay), a simple, training-free early-stopping framework for multimodal multi-agent reasoning based on two core designs. First, we introduce Readout-Driven Early Stopping: while the initial agent is reasoning, we periodically read out its tentative answer and stop generation early once the prediction stabilizes with high confidence. Second, we design Context-Reset Visual Relay: when early readouts fail to stabilize with high confidence, we stop the initial agent early and reset the context by discarding its unfinished reasoning text. We then crop task-relevant image regions and pass only the visual information to a verification agent to re-evaluate the question in a clean context. Coupling these two designs saves tokens on easy questions and prevents error propagation on hard ones. Across MMStar, MathVista, and WeMath on Qwen3-VL-8B and 4B, RELAY improves accuracy by 3.1% and 3.4% over LatentMAS, reduces token cost by 24%-39%, and accelerates inference by 1.6x, while generalizing to text-based tasks without performance degradation.

==> results.tex <==
% Frozen numerical results for RELAY (pruned to active keys).
\makeatletter
\newcommand{\res}[1]{\csname res@#1\endcsname}
\expandafter\def\csname res@acc_always\endcsname{74.6}
\expandafter\def\csname res@acc_always_mathvista\endcsname{82.9}
\expandafter\def\csname res@acc_always_mmstar\endcsname{70.3}
\expandafter\def\csname res@acc_always_wemath\endcsname{74.1}
\expandafter\def\csname res@acc_c1\endcsname{73.5}
\expandafter\def\csname res@acc_c1_mathvista\endcsname{82.9}
\expandafter\def\csname res@acc_c1_mmstar\endcsname{68.4}
\expandafter\def\csname res@acc_c1_wemath\endcsname{73.3}
\expandafter\def\csname res@acc_cotg\endcsname{73.9}
\expandafter\def\csname res@acc_lmas\endcsname{70.3}
\expandafter\def\csname res@acc_lmas_mathvista\endcsname{80.8}
\expandafter\def\csname res@acc_lmas_mmstar\endcsname{65.0}
\expandafter\def\csname res@acc_lmas_wemath\endcsname{69.8}
\expandafter\def\csname res@acc_ours\endcsname{73.5}
\expandafter\def\csname res@acc_ours_mathvista\endcsname{81.8}
\expandafter\def\csname res@acc_ours_mmstar\endcsname{68.3}
\expandafter\def\csname res@acc_ours_wemath\endcsname{74.0}
\expandafter\def\csname res@acc_pj\endcsname{71.2}
\expandafter\def\csname res@acc_pj_mathvista\endcsname{81.4}
\expandafter\def\csname res@acc_pj_mmstar\endcsname{65.8}
\expandafter\def\csname res@acc_pj_wemath\endcsname{70.8}
\expandafter\def\csname res@acc_sc3\endcsname{74.7}
\expandafter\def\csname res@acc_si\endcsname{74.0}
\expandafter\def\csname res@acc_si_mathvista\endcsname{83.6}
\expandafter\def\csname res@acc_si_mmstar\endcsname{68.5}
\expandafter\def\csname res@acc_si_wemath\endcsname{74.0}
\expandafter\def\csname res@acc_single\endcsname{72.4}
\expandafter\def\csname res@acc_single_mathvista\endcsname{81.8}
\expandafter\def\csname res@acc_single_mmstar\endcsname{67.4}
\expandafter\def\csname res@acc_single_wemath\endcsname{72.1}
\expandafter\def\csname res@acc_tm\endcsname{68.2}
\expandafter\def\csname res@acc_tm_mathvista\endcsname{81.1}
\expandafter\def\csname res@acc_tm_mmstar\endcsname{62.7}
\expandafter\def\csname res@acc_tm_wemath\endcsname{66.4}
\expandafter\def\csname res@fr_acc_always\endcsname{74.6}
\expandafter\def\csname res@fr_acc_c1\endcsname{73.5}
\expandafter\def\csname res@fr_acc_cap\endcsname{74.3}
\expandafter\def\csname res@fr_acc_cut1024\endcsname{73.9}
\expandafter\def\csname res@fr_acc_dev\endcsname{73.5}
\expandafter\def\csname res@fr_acc_frozen\endcsname{73.5}
\expandafter\def\csname res@fr_out_dev\endcsname{603}
\expandafter\def\csname res@fresh_solve_share\endcsname{16.3}
\expandafter\def\csname res@gr_acc_lmas\endcsname{72.5}
\expandafter\def\csname res@gr_acc_pcrj\endcsname{73.1}
\expandafter\def\csname res@gr_acc_pj\endcsname{73.0}
\expandafter\def\csname res@gr_dec_lmas\endcsname{570}
\expandafter\def\csname res@gr_dec_pcrj\endcsname{583}
\expandafter\def\csname res@gr_dec_pj\endcsname{580}
\expandafter\def\csname res@h1_pt\endcsname{3.1}
\expandafter\def\csname res@h3_pt\endcsname{1.9}
\expandafter\def\csname res@m2_acc_lmas\endcsname{69.3}
\expandafter\def\csname res@m2_acc_lmas_mathvista\endcsname{79.6}
\expandafter\def\csname res@m2_acc_lmas_mmstar\endcsname{62.7}
\expandafter\def\csname res@m2_acc_lmas_wemath\endcsname{69.9}
\expandafter\def\csname res@m2_acc_ours\endcsname{72.7}
\expandafter\def\csname res@m2_acc_ours_mathvista\endcsname{83.4}
\expandafter\def\csname res@m2_acc_ours_mmstar\endcsname{63.7}
\expandafter\def\csname res@m2_acc_ours_wemath\endcsname{75.5}
\expandafter\def\csname res@m2_acc_pj\endcsname{68.6}
\expandafter\def\csname res@m2_acc_pj_mathvista\endcsname{77.8}
\expandafter\def\csname res@m2_acc_pj_mmstar\endcsname{62.6}
\expandafter\def\csname res@m2_acc_pj_wemath\endcsname{69.4}
\expandafter\def\csname res@m2_acc_sc3\endcsname{74.6}
\expandafter\def\csname res@m2_acc_single\endcsname{70.8}
\expandafter\def\csname res@m2_acc_single_mathvista\endcsname{81.3}
\expandafter\def\csname res@m2_acc_single_mmstar\endcsname{65.2}
\expandafter\def\csname res@m2_acc_single_wemath\endcsname{70.6}
\expandafter\def\csname res@m2_gr_acc_lmas\endcsname{71.7}
\expandafter\def\csname res@m2_gr_acc_pcrj\endcsname{71.1}
\expandafter\def\csname res@m2_gr_acc_pj\endcsname{71.8}
\expandafter\def\csname res@m2_gr_dec_lmas\endcsname{556}
\expandafter\def\csname res@m2_gr_dec_pcrj\endcsname{550}
\expandafter\def\csname res@m2_gr_dec_pj\endcsname{527}
\expandafter\def\csname res@m2_h5_pt\endcsname{3.4}
\expandafter\def\csname res@m2_out_lmas\endcsname{723}
\expandafter\def\csname res@m2_out_ours\endcsname{441}
\expandafter\def\csname res@m2_out_pj\endcsname{723}
\expandafter\def\csname res@m2_out_sc3\endcsname{1{,}437}
\expandafter\def\csname res@m2_out_single\endcsname{580}
\expandafter\def\csname res@n_confirm\endcsname{921}
\expandafter\def\csname res@n_mathvista\endcsname{201}
\expandafter\def\csname res@n_mmstar\endcsname{354}
\expandafter\def\csname res@n_wemath\endcsname{366}
\expandafter\def\csname res@out_always\endcsname{937}
\expandafter\def\csname res@out_c1\endcsname{564}
\expandafter\def\csname res@out_cotg\endcsname{596}
\expandafter\def\csname res@out_lmas\endcsname{689}
\expandafter\def\csname res@out_ours\endcsname{526}
\expandafter\def\csname res@out_pj\endcsname{706}
\expandafter\def\csname res@out_sc3\endcsname{1{,}788}
\expandafter\def\csname res@out_si\endcsname{647}
\expandafter\def\csname res@out_single\endcsname{529}
\expandafter\def\csname res@out_tm\endcsname{1{,}373}
\expandafter\def\csname res@path_acc_finish\endcsname{77.9}
\expandafter\def\csname res@path_acc_settled\endcsname{78.8}
\expandafter\def\csname res@path_share_finish\endcsname{47.3}
\expandafter\def\csname res@path_share_rstop\endcsname{0.4}
\expandafter\def\csname res@path_share_settled\endcsname{28.0}
\expandafter\def\csname res@st_acc_m40\endcsname{70.5}
\expandafter\def\csname res@st_acc_m80\endcsname{70.6}
\expandafter\def\csname res@st_dec_m40\endcsname{767}
\expandafter\def\csname res@st_dec_m80\endcsname{854}
\expandafter\def\csname res@t_lmas\endcsname{93.1}
\expandafter\def\csname res@t_lmas_arcc\endcsname{92.4}
\expandafter\def\csname res@t_lmas_arce\endcsname{95.7}
\expandafter\def\csname res@t_lmas_gsm\endcsname{91.2}
\expandafter\def\csname res@t_ours\endcsname{95.0}
\expandafter\def\csname res@t_ours_arcc\endcsname{94.1}
\expandafter\def\csname res@t_ours_arce\endcsname{98.6}
\expandafter\def\csname res@t_ours_gsm\endcsname{92.2}
\expandafter\def\csname res@t_out_lmas\endcsname{637}
\expandafter\def\csname res@t_out_ours\endcsname{508}
\expandafter\def\csname res@t_out_single\endcsname{740}
\expandafter\def\csname res@t_out_tm\endcsname{2{,}277}
\expandafter\def\csname res@t_single\endcsname{93.3}
\expandafter\def\csname res@t_single_arcc\endcsname{91.8}
\expandafter\def\csname res@t_single_arce\endcsname{97.9}
\expandafter\def\csname res@t_single_gsm\endcsname{90.3}
\expandafter\def\csname res@t_tm\endcsname{96.2}
\expandafter\def\csname res@t_tm_arcc\endcsname{95.0}
\expandafter\def\csname res@t_tm_arce\endcsname{99.0}
\expandafter\def\csname res@t_tm_gsm\endcsname{94.6}
\expandafter\def\csname res@tr_lmas_arcc\endcsname{94.4}
\expandafter\def\csname res@tr_lmas_arce\endcsname{98.8}
\expandafter\def\csname res@tr_lmas_gsm\endcsname{93.8}
\expandafter\def\csname res@tr_single_arcc\endcsname{91.0}
\expandafter\def\csname res@tr_single_arce\endcsname{95.6}
\expandafter\def\csname res@tr_single_gsm\endcsname{81.1}
\expandafter\def\csname res@tr_tm_arcc\endcsname{94.6}
\expandafter\def\csname res@tr_tm_arce\endcsname{99.1}
\expandafter\def\csname res@tr_tm_gsm\endcsname{92.3}
\expandafter\def\csname res@w_all_c1_acc\endcsname{58.7}
\expandafter\def\csname res@w_all_c1_out\endcsname{1{,}499}
\expandafter\def\csname res@w_all_ours_acc\endcsname{58.6}
\expandafter\def\csname res@w_all_ours_out\endcsname{1{,}342}
\expandafter\def\csname res@w_all_share\endcsname{24.2}
\expandafter\def\csname res@w_glance_c1_acc\endcsname{63.5}
\expandafter\def\csname res@w_glance_c1_out\endcsname{1{,}466}
\expandafter\def\csname res@w_glance_ours_acc\endcsname{65.3}
\expandafter\def\csname res@w_glance_ours_out\endcsname{589}
\expandafter\def\csname res@w_glance_share\endcsname{7.9}
\expandafter\def\csname res@x_c512_acc\endcsname{73.7}
\expandafter\def\csname res@x_c512_out\endcsname{533}
\expandafter\def\csname res@x_confm_acc\endcsname{74.2}
\expandafter\def\csname res@x_confm_out\endcsname{710}
\expandafter\def\csname res@x_cut_acc\endcsname{71.8}
\expandafter\def\csname res@x_cut_loss_pt\endcsname{1.7}
\expandafter\def\csname res@x_cut_out\endcsname{332}
\makeatother

